Communicative On-Policy Distillation: Distilling Black-Box Teacher Capabilities through Communication for Long-Horizon Tasks

On-policy distillation (OPD) is a powerful paradigm for improving language-model agents on long-horizon tasks, yet its conventional formulation relies on teacher logits that text-only black- box models do not expose. To address this limitation, we introduce Communicative On-Policy Distillation (COPD), which uses natural-language communication as a medium for distilling a stronger model's capabilities into a smaller student. During task execution, the student au- tonomously decides when to consult a black-box teacher and formulates open-ended natural- language requests without predefined question templates or intervention schedules. Successful student-teacher interactions are retained as privileged references to supervise fresh adviser-free student rollouts through on-policy self-distillation, jointly with task-reward reinforcement learning. On CAMG-II, COPD achieves 2.46 times the gain of the strongest black-box OPD baseline. The capabilities it learns through communication generalize to Terminal-Bench 2.1 and SWE-Bench Pro V2, improving task success without adviser access.

==> tables/hyperparameter_values.tex <==
% Generated from evidence/hyperparameter_reference.json; do not edit numeric cells.
\newcommand{\HPUpdates}{100}
\newcommand{\HPEpisodes}{64}
\newcommand{\HPExposures}{6,400}
\newcommand{\HPDomainExposures}{1,280}
\newcommand{\HPSequence}{98,304}
\newcommand{\HPPrompt}{65,536}
\newcommand{\HPResponse}{32,768}


==> tables/reward_contract.tex <==
% Rows follow the reward contracts implemented by the released environment packages:
% webshop six-session goal reward, agentenv-swesmith REWARD_CONTRACT, agentenv-openmle-fast
% soft-floor contract, agentenv-agentgeneral rubric_outcome_finish_only_v2, and
% agentenv webdev_vision_rubric_outcome_finish_only_v1.
\begin{table*}[!t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.115\textwidth}>{\raggedright\arraybackslash}p{0.84\textwidth}@{}}
\toprule
\textbf{Environment} & \textbf{Reward} \\
\midrule
Shop & $r_t=\tfrac{1}{7}$ per correct purchase of the session target under the cumulative budget. A
wrong purchase pays $-0.5$ and terminates the episode with earlier payments retained. Success requires
the full six-session sequence. \\
Coding & $R=\mathbf{1}[\text{hidden tests pass on the submitted repository change}]$ at the submission
sentinel. The penalty is $r_t=-0.01$ per recoverable invalid action and at horizon failure. \\
AutoResearch & $R=\max(0,\,m)+0.05\,\mathbf{1}[\text{first execution}]+0.10\,\mathbf{1}[\text{first
validation}]$, where $m$ is the private grader's native-metric score of the submitted file and milestone
payments are capped at $0.15$ per episode. The penalty is $r_t=-0.01$ at action-budget exhaustion or wall-clock
termination, and invalid submissions pay $0$. \\
General & $R=\mathbf{w}^{\top}\mathbf{r}$, a weighted rubric over the final answer, delivered files,
and post-action system state, paid once at finish with required rule checks as gates. The reward is $r_t=-0.1$ per
invalid action and $-0.01$ when the budget is exhausted without a submission. \\
Visual & $R=\mathrm{mean}(r_{\mathrm{rubric}},\,r_{\mathrm{fulfilment}},\,r_{\mathrm{assets}})$, an
absolute rubric over screenshots of the delivered page at finish (layout, typography, color,
whitespace, content), averaged with query fulfilment and asset quality. Invalid actions pay $0$. \\
\bottomrule
\end{tabular}
\caption{\textbf{Task rewards.}}
\label{tab:reward-contract}
\end{table*}


==> tables/training_config.tex <==
% Generated from evidence/hyperparameter_reference.json; do not edit numeric cells.
\begin{table*}[!t]
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.06}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.19\textwidth}>{\raggedright\arraybackslash}p{0.43\textwidth}>{\raggedright\arraybackslash}p{\dimexpr0.38\textwidth-12pt\relax}@{}}
\toprule
Group & Hyperparameter & Value \\
\midrule
Models & Student (full parameters) & Qwen3.5-4B / Qwen3.5-9B \\
 & Critic initialization & Same student initialization \\
\midrule
Objective & Task-PPO loss / learned critic & On / On \\
 & PPO clip & 0.2 \\
 & Value clip & 0.5 \\
 & Discount $\gamma$ / GAE $\lambda$ & 1 / 1 \\
 & Entropy / auxiliary reference KL coefficient & 0 / 0 \\
\midrule
Schedule & Learner rounds & 100 \\
 & Episodes per learner round & 64 \\
 & Passes per episode batch & 1 \\
 & Domain mixture & Equal, balanced interleaving \\
 & Rollout / FSDP / data-loader seeds & 42 / 42 / 42 \\
\midrule
Optimizer & Optimizer & AdamW \\
 & Actor learning rate & $10^{-6}$ (constant) \\
 & Critic learning rate & $10^{-5}$ (constant) \\
 & AdamW $(\beta_1,\beta_2)$ & $(0.9,0.999)$ \\
 & AdamW $\epsilon$ & $10^{-8}$ \\
 & Weight decay & 0.01 \\
 & Warmup updates & 0 \\
 & Gradient norm limit & 1.0 \\
\midrule
Batching & Responses per GPU microbatch & $\leq 8$ \\
 & Tokens per GPU microbatch & $\leq 98,304$ \\
 & Rows per optimizer minibatch & 510 \\
 & Gradient accumulation & One step per actor or critic optimizer minibatch \\
\midrule
Runtime & Precision / sharding & BF16 / FSDP2 \\
 & Gradient checkpointing & On \\
 & Weight publication & Every 1 learner round \\
\midrule
Decoding & Temperature / top-$p$ & 1 / 1 \\
 & Sampling top-$k$ / responses per invocation & Disabled / 1 \\
\midrule
Sequence & Prompt + sampled response & 98,304 tokens \\
 & Prompt ceiling & 65,536 tokens \\
 & Response ceiling & 32,768 tokens \\
 & Route observation envelope & 8,192 (Shop, Coding, AutoResearch), 12,288 (General, Visual) tokens \\
\bottomrule
\end{tabular}
\caption{\textbf{Training configuration.}}
\label{tab:training-common}
\end{table*}

